JADES: Resolving the Stellar Component and Filamentary Overdense Environment of HST-Dark Submillimeter Galaxy HDF850.1 at $z=5.18$

HDF850.1 is the brightest submillimeter galaxy (SMG) in the Hubble Deep Field. It is known as a heavily dust-obscured star-forming galaxy embedded in an overdense environment at $z = 5.18$. With nine-band NIRCam images at 0.8-5.0 $\mu$m obtained through the JWST Advanced Deep Extragalactic Survey (JADES), we detect and resolve the rest-frame UV-optical counterpart of HDF850.1, which splits into two components because of heavy dust obscuration in the center. The southern component leaks UV and H$\alpha$ photons, bringing the galaxy $\sim$100 times above the empirical relation between infrared excess and UV continuum slope (IRX-$\beta_\mathrm{UV}$). The northern component is higher in dust attenuation and thus fainter in UV and H$\alpha$ surface brightness. We construct a spatially resolved dust attenuation map from the NIRCam images, well matched with the dust continuum emission obtained through millimeter interferometry. The whole system hosts a stellar mass of $10^{10.8\pm0.1}\,\mathrm{M}_\odot$ and star-formation rate of $10^{2.8\pm0.2}\,\mathrm{M}_\odot\,\mathrm{yr}^{-1}$, placing the galaxy at the massive end of the star-forming main sequence at this epoch. We further confirm that HDF850.1 resides in a complex overdense environment at $z=5.17-5.30$, which hosts another luminous SMG at $z=5.30$ (GN10). The filamentary structures of the overdensity are characterized by 109 H$\alpha$-emitting galaxies confirmed through NIRCam slitless spectroscopy at 3.9-5 $\mu$m, of which only eight were known before the JWST observations. Given the existence of a similar galaxy overdensity in the GOODS-S field, our results suggest that $50\pm20$% of the cosmic star formation at $z=5.1-5.5$ occur in protocluster environments.

==> 04f_further.tex <==
\subsection{Further Discussion}
\label{ss:04f_further}

Massive galaxies including SMGs and quasar-host galaxies in the high-redshift Universe have been long suggested to form in massive dark matter halos \citep[e.g.,][]{springel05}. 
Therefore, it is a natural consequence that massive SMGs at high redshifts preferentially trace galaxy overdensities, as has been widely reported in the literature, such as the  SMGs in the SSA\,22 protocluster \citep[$z=3.1$;][]{umehata19}, the DRC \citep[$z=4.0$;][]{oteo18}, GN20 \citep[$z=4.05$;][]{daddi09b}, the AS2COS0001 system \citep[$z=4.6$;][]{mitsuhashi20} and AzTEC-3 \citep[$z=5.3$;][]{guaita22}, etc.

With the advent of JWST, it is now possible to study high-redshift SMGs and their environments through rest-frame optical spectroscopy with NIRCam WFSS and NIRSpec MSA.
This is important for the studies of the environment of high-redshift SMGs (or other massive galaxies) especially at $z\gtrsim6$ where the success rate of ground-based \lya\ detection declines sharply because of the increasing neutral fraction of IGM (see review in \citealt{stark16}).
Ground-based millimeter interferometry can be helpful in confirming gas-rich protocluster members through CO, \cii\ or other far-IR coolants \citep[e.g.,][]{decarli17,meyer22}, but the small primary beam size (e.g., $\sim$20\arcsec\ for ALMA at 1\,mm) limits the efficiency in wide-field surveys.

Specifically, with JWST, the NIRCam WFSS mode has been proven to be highly efficient in mapping galaxy overdensities around the Epoch of Reionization \citep[e.g.,][]{kashino22,matthee22,helton23,wang23}. 
The NIRCam WFSS does not require pre-selection of targets or suffer from slit loss, and therefore it is able to provide unbiased, highly complete line-flux-limited (i.e., complete in SFR if the \ha\ line is used as the tracer, assuming negligible dust attenuation) samples of star-forming galaxies in the overdense environment.
Even considering the high dust attenuation seen with SMGs like HDF850.1, the NIRCam WFSS is also able to detect the unobscured portion of \ha\ emission from these galaxies as long as they enter the redshift window (e.g., $z=4.9-6.5$ for \ha\ with NIRCam F444W filter).
This promises highly complete redshift surveys of dusty star-forming galaxies around the epoch of reionization, greatly enhancing the accuracy of dust-obscured SFR density measurements at $z\gtrsim4$ (e.g., \citealt{gruppioni20,casey21,fujimoto23}) through direct and spectroscopically complete infrared luminosity function measurements.
On the other hand, with higher sensitivity because of lower sky background, the NIRSpec MSA can be more advantageous in follow-up observations of confirmed overdensity members, characterizing the kinematics and physical properties of the interstellar medium (e.g., excitation and metal enrichment history) of these galaxies and investigating the environmental effects in the early Universe. 

==> 10b_apd_figset.tex <==
\figsetstart
\figsetnum{A1}
\figsettitle{NIRCam images, 2D and 1D grism spectra of 140 spectroscopically confirmed galaxies at $z = 5.1 - 5.5$.}

\figsetgrpstart
\figsetgrpnum{A1.1}
\figsetgrptitle{JADES-GN-189.06961+62.27808}
\figsetplot{figures/aastex_specfigs/spec_ID15920.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.06961+62.27808 at $z=5.115$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.2}
\figsetgrptitle{JADES-GN-189.09098+62.27600}
\figsetplot{figures/aastex_specfigs/spec_ID15254.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.09098+62.27600 at $z=5.126$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.3}
\figsetgrptitle{JADES-GN-189.08706+62.26738}
\figsetplot{figures/aastex_specfigs/spec_ID12781.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.08706+62.26738 at $z=5.131$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.4}
\figsetgrptitle{JADES-GN-189.15434+62.24967}
\figsetplot{figures/aastex_specfigs/spec_ID8233.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.15434+62.24967 at $z=5.141$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.5}
\figsetgrptitle{JADES-GN-189.08801+62.26874}
\figsetplot{figures/aastex_specfigs/spec_ID30132.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.08801+62.26874 at $z=5.141$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.6}
\figsetgrptitle{JADES-GN-189.06429+62.27429}
\figsetplot{figures/aastex_specfigs/spec_ID14693.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.06429+62.27429 at $z=5.145$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.7}
\figsetgrptitle{JADES-GN-189.11978+62.22501}
\figsetplot{figures/aastex_specfigs/spec_ID1167.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.11978+62.22501 at $z=5.172$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.8}
\figsetgrptitle{JADES-GN-189.20867+62.20743}
\figsetplot{figures/aastex_specfigs/spec_ID79357.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.20867+62.20743 at $z=5.172$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.9}
\figsetgrptitle{JADES-GN-189.13071+62.22752}
\figsetplot{figures/aastex_specfigs/spec_ID1698.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.13071+62.22752 at $z=5.173$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.10}
\figsetgrptitle{JADES-GN-189.14055+62.22303}
\figsetplot{figures/aastex_specfigs/spec_ID847.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.14055+62.22303 at $z=5.175$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.11}
\figsetgrptitle{JADES-GN-189.24900+62.21834}
\figsetplot{figures/aastex_specfigs/spec_ID62309.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.24900+62.21834 at $z=5.175$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.12}
\figsetgrptitle{JADES-GN-189.11531+62.23411}
\figsetplot{figures/aastex_specfigs/spec_ID3205.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.11531+62.23411 at $z=5.176$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.13}
\figsetgrptitle{JADES-GN-189.14948+62.22198}
\figsetplot{figures/aastex_specfigs/spec_ID24702.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.14948+62.22198 at $z=5.177$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.14}
\figsetgrptitle{JADES-GN-189.13328+62.22751}
\figsetplot{figures/aastex_specfigs/spec_ID1674.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.13328+62.22751 at $z=5.178$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.15}
\figsetgrptitle{JADES-GN-189.11761+62.24433}
\figsetplot{figures/aastex_specfigs/spec_ID6357.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.11761+62.24433 at $z=5.178$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.16}
\figsetgrptitle{JADES-GN-189.13261+62.22674}
\figsetplot{figures/aastex_specfigs/spec_ID1511.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.13261+62.22674 at $z=5.179$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.17}
\figsetgrptitle{JADES-GN-189.12590+62.22916}
\figsetplot{figures/aastex_specfigs/spec_ID2030.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.12590+62.22916 at $z=5.180$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.18}
\figsetgrptitle{JADES-GN-189.23848+62.20022}
\figsetplot{figures/aastex_specfigs/spec_ID55988.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.23848+62.20022 at $z=5.180$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.19}
\figsetgrptitle{JADES-GN-189.13539+62.22536}
\figsetplot{figures/aastex_specfigs/spec_ID1239.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.13539+62.22536 at $z=5.180$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.20}
\figsetgrptitle{JADES-GN-189.24868+62.24843}
\figsetplot{figures/aastex_specfigs/spec_ID27712.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.24868+62.24843 at $z=5.182$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.21}
\figsetgrptitle{JADES-GN-189.11695+62.22208}
\figsetplot{figures/aastex_specfigs/spec_ID24719.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.11695+62.22208 at $z=5.183$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.22}
\figsetgrptitle{JADES-GN-189.18074+62.28224}
\figsetplot{figures/aastex_specfigs/spec_ID17070.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.18074+62.28224 at $z=5.183$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.23}
\figsetgrptitle{JADES-GN-189.21582+62.18648}
\figsetplot{figures/aastex_specfigs/spec_ID75221.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.21582+62.18648 at $z=5.183$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.24}
\figsetgrptitle{JADES-GN-189.15632+62.21000}
\figsetplot{figures/aastex_specfigs/spec_ID59412.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.15632+62.21000 at $z=5.183$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.25}
\figsetgrptitle{JADES-GN-189.20968+62.20726}
\figsetplot{figures/aastex_specfigs/spec_ID79349.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.20968+62.20726 at $z=5.183$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.26}
\figsetgrptitle{JADES-GN-189.19199+62.22137}
\figsetplot{figures/aastex_specfigs/spec_ID63227.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.19199+62.22137 at $z=5.184$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.27}
\figsetgrptitle{JADES-GN-189.27453+62.20191}
\figsetplot{figures/aastex_specfigs/spec_ID56618.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.27453+62.20191 at $z=5.184$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.28}
\figsetgrptitle{JADES-GN-189.23869+62.21371}
\figsetplot{figures/aastex_specfigs/spec_ID80616.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.23869+62.21371 at $z=5.184$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.29}
\figsetgrptitle{JADES-GN-189.20777+62.21324}
\figsetplot{figures/aastex_specfigs/spec_ID80255.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.20777+62.21324 at $z=5.184$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.30}
\figsetgrptitle{JADES-GN-189.27348+62.22835}
\figsetplot{figures/aastex_specfigs/spec_ID82359.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.27348+62.22835 at $z=5.184$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.31}
\figsetgrptitle{JADES-GN-189.23137+62.25908}
\figsetplot{figures/aastex_specfigs/spec_ID29046.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.23137+62.25908 at $z=5.185$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.32}
\figsetgrptitle{JADES-GN-189.19472+62.18163}
\figsetplot{figures/aastex_specfigs/spec_ID74297.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.19472+62.18163 at $z=5.185$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.33}
\figsetgrptitle{JADES-GN-189.20629+62.21533}
\figsetplot{figures/aastex_specfigs/spec_ID80875.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.20629+62.21533 at $z=5.185$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.34}
\figsetgrptitle{JADES-GN-189.16011+62.25755}
\figsetplot{figures/aastex_specfigs/spec_ID10371.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.16011+62.25755 at $z=5.186$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.35}
\figsetgrptitle{JADES-GN-189.23124+62.25913}
\figsetplot{figures/aastex_specfigs/spec_ID29048.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.23124+62.25913 at $z=5.186$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.36}
\figsetgrptitle{JADES-GN-189.20621+62.25295}
\figsetplot{figures/aastex_specfigs/spec_ID9229.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.20621+62.25295 at $z=5.186$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.37}
\figsetgrptitle{JADES-GN-189.23103+62.25912}
\figsetplot{figures/aastex_specfigs/spec_ID29047.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.23103+62.25912 at $z=5.186$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.38}
\figsetgrptitle{JADES-GN-189.20293+62.20467}
\figsetplot{figures/aastex_specfigs/spec_ID78773.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.20293+62.20467 at $z=5.186$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.39}
\figsetgrptitle{JADES-GN-189.23545+62.22043}
\figsetplot{figures/aastex_specfigs/spec_ID62955.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.23545+62.22043 at $z=5.186$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.40}
\figsetgrptitle{JADES-GN-189.21754+62.26311}
\figsetplot{figures/aastex_specfigs/spec_ID11679.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.21754+62.26311 at $z=5.187$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.41}
\figsetgrptitle{JADES-GN-189.16961+62.18386}
\figsetplot{figures/aastex_specfigs/spec_ID74777.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.16961+62.18386 at $z=5.187$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.42}
\figsetgrptitle{JADES-GN-189.22121+62.21652}
\figsetplot{figures/aastex_specfigs/spec_ID61712.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.22121+62.21652 at $z=5.187$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.43}
\figsetgrptitle{JADES-GN-189.21680+62.19577}
\figsetplot{figures/aastex_specfigs/spec_ID77112.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.21680+62.19577 at $z=5.187$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.44}
\figsetgrptitle{JADES-GN-189.17570+62.18671}
\figsetplot{figures/aastex_specfigs/spec_ID75274.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.17570+62.18671 at $z=5.187$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.45}
\figsetgrptitle{JADES-GN-189.21809+62.26809}
\figsetplot{figures/aastex_specfigs/spec_ID12941.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.21809+62.26809 at $z=5.188$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.46}
\figsetgrptitle{JADES-GN-189.20512+62.26072}
\figsetplot{figures/aastex_specfigs/spec_ID11050.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.20512+62.26072 at $z=5.188$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.47}
\figsetgrptitle{JADES-GN-189.23482+62.25750}
\figsetplot{figures/aastex_specfigs/spec_ID28887.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.23482+62.25750 at $z=5.188$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.48}
\figsetgrptitle{JADES-GN-189.16549+62.30689}
\figsetplot{figures/aastex_specfigs/spec_ID35508.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.16549+62.30689 at $z=5.188$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.49}
\figsetgrptitle{JADES-GN-189.20744+62.17914}
\figsetplot{figures/aastex_specfigs/spec_ID73852.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.20744+62.17914 at $z=5.188$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.50}
\figsetgrptitle{JADES-GN-189.19692+62.28451}
\figsetplot{figures/aastex_specfigs/spec_ID17807.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.19692+62.28451 at $z=5.188$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.51}
\figsetgrptitle{JADES-GN-189.24689+62.20341}
\figsetplot{figures/aastex_specfigs/spec_ID78732.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.24689+62.20341 at $z=5.189$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.52}
\figsetgrptitle{JADES-GN-189.23078+62.26355}
\figsetplot{figures/aastex_specfigs/spec_ID11804.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.23078+62.26355 at $z=5.189$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.53}
\figsetgrptitle{JADES-GN-189.16658+62.30560}
\figsetplot{figures/aastex_specfigs/spec_ID23340.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.16658+62.30560 at $z=5.192$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.54}
\figsetgrptitle{JADES-GN-189.10025+62.23082}
\figsetplot{figures/aastex_specfigs/spec_ID25435.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.10025+62.23082 at $z=5.193$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.55}
\figsetgrptitle{JADES-GN-189.13667+62.29864}
\figsetplot{figures/aastex_specfigs/spec_ID22131.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.13667+62.29864 at $z=5.194$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.56}
\figsetgrptitle{JADES-GN-189.10034+62.23089}
\figsetplot{figures/aastex_specfigs/spec_ID25436.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.10034+62.23089 at $z=5.195$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.57}
\figsetgrptitle{JADES-GN-189.11534+62.29500}
\figsetplot{figures/aastex_specfigs/spec_ID34445.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.11534+62.29500 at $z=5.199$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.58}
\figsetgrptitle{JADES-GN-189.22478+62.22575}
\figsetplot{figures/aastex_specfigs/spec_ID64405.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.22478+62.22575 at $z=5.201$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.59}
\figsetgrptitle{JADES-GN-189.25771+62.22433}
\figsetplot{figures/aastex_specfigs/spec_ID81996.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.25771+62.22433 at $z=5.205$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.60}
\figsetgrptitle{JADES-GN-189.08401+62.26984}
\figsetplot{figures/aastex_specfigs/spec_ID13426.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.08401+62.26984 at $z=5.205$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.61}
\figsetgrptitle{JADES-GN-189.08302+62.26969}
\figsetplot{figures/aastex_specfigs/spec_ID13368.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.08302+62.26969 at $z=5.206$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.62}
\figsetgrptitle{JADES-GN-189.24659+62.21494}
\figsetplot{figures/aastex_specfigs/spec_ID80685.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.24659+62.21494 at $z=5.208$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.63}
\figsetgrptitle{JADES-GN-189.28294+62.20472}
\figsetplot{figures/aastex_specfigs/spec_ID57629.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.28294+62.20472 at $z=5.211$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.64}
\figsetgrptitle{JADES-GN-189.26381+62.22539}
\figsetplot{figures/aastex_specfigs/spec_ID64298.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.26381+62.22539 at $z=5.214$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.65}
\figsetgrptitle{JADES-GN-189.23731+62.19031}
\figsetplot{figures/aastex_specfigs/spec_ID52302.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.23731+62.19031 at $z=5.218$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.66}
\figsetgrptitle{JADES-GN-189.26554+62.19931}
\figsetplot{figures/aastex_specfigs/spec_ID77853.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.26554+62.19931 at $z=5.220$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.67}
\figsetgrptitle{JADES-GN-189.26569+62.19927}
\figsetplot{figures/aastex_specfigs/spec_ID77852.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.26569+62.19927 at $z=5.220$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.68}
\figsetgrptitle{JADES-GN-189.26541+62.19937}
\figsetplot{figures/aastex_specfigs/spec_ID77854.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.26541+62.19937 at $z=5.220$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.69}
\figsetgrptitle{JADES-GN-189.26502+62.19955}
\figsetplot{figures/aastex_specfigs/spec_ID77908.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.26502+62.19955 at $z=5.221$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.70}
\figsetgrptitle{JADES-GN-189.24928+62.20532}
\figsetplot{figures/aastex_specfigs/spec_ID79046.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.24928+62.20532 at $z=5.221$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.71}
\figsetgrptitle{JADES-GN-189.26510+62.19963}
\figsetplot{figures/aastex_specfigs/spec_ID77909.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.26510+62.19963 at $z=5.222$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.72}
\figsetgrptitle{JADES-GN-189.28549+62.20682}
\figsetplot{figures/aastex_specfigs/spec_ID79313.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.28549+62.20682 at $z=5.222$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.73}
\figsetgrptitle{JADES-GN-189.25382+62.19701}
\figsetplot{figures/aastex_specfigs/spec_ID77346.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.25382+62.19701 at $z=5.223$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.74}
\figsetgrptitle{JADES-GN-189.26643+62.20915}
\figsetplot{figures/aastex_specfigs/spec_ID79689.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.26643+62.20915 at $z=5.223$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.75}
\figsetgrptitle{JADES-GN-189.30578+62.21089}
\figsetplot{figures/aastex_specfigs/spec_ID59718.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.30578+62.21089 at $z=5.223$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.76}
\figsetgrptitle{JADES-GN-189.28570+62.20676}
\figsetplot{figures/aastex_specfigs/spec_ID79312.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.28570+62.20676 at $z=5.223$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.77}
\figsetgrptitle{JADES-GN-189.25565+62.19426}
\figsetplot{figures/aastex_specfigs/spec_ID53780.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.25565+62.19426 at $z=5.224$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.78}
\figsetgrptitle{JADES-GN-189.26168+62.19490}
\figsetplot{figures/aastex_specfigs/spec_ID77004.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.26168+62.19490 at $z=5.224$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.79}
\figsetgrptitle{JADES-GN-189.25428+62.20769}
\figsetplot{figures/aastex_specfigs/spec_ID58669.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.25428+62.20769 at $z=5.225$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.80}
\figsetgrptitle{JADES-GN-189.19396+62.17536}
\figsetplot{figures/aastex_specfigs/spec_ID46918.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.19396+62.17536 at $z=5.226$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.81}
\figsetgrptitle{JADES-GN-189.26137+62.20801}
\figsetplot{figures/aastex_specfigs/spec_ID79520.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.26137+62.20801 at $z=5.227$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.82}
\figsetgrptitle{JADES-GN-189.24913+62.20519}
\figsetplot{figures/aastex_specfigs/spec_ID79043.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.24913+62.20519 at $z=5.227$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.83}
\figsetgrptitle{JADES-GN-189.15686+62.30453}
\figsetplot{figures/aastex_specfigs/spec_ID35355.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.15686+62.30453 at $z=5.242$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.84}
\figsetgrptitle{JADES-GN-189.09366+62.23480}
\figsetplot{figures/aastex_specfigs/spec_ID3394.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.09366+62.23480 at $z=5.245$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.85}
\figsetgrptitle{JADES-GN-189.13369+62.24499}
\figsetplot{figures/aastex_specfigs/spec_ID6609.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.13369+62.24499 at $z=5.257$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.86}
\figsetgrptitle{JADES-GN-189.14244+62.28573}
\figsetplot{figures/aastex_specfigs/spec_ID33043.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.14244+62.28573 at $z=5.264$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.87}
\figsetgrptitle{JADES-GN-189.14260+62.28570}
\figsetplot{figures/aastex_specfigs/spec_ID33042.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.14260+62.28570 at $z=5.264$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.88}
\figsetgrptitle{JADES-GN-189.12617+62.23717}
\figsetplot{figures/aastex_specfigs/spec_ID26141.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.12617+62.23717 at $z=5.266$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.89}
\figsetgrptitle{JADES-GN-189.11794+62.23552}
\figsetplot{figures/aastex_specfigs/spec_ID3608.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.11794+62.23552 at $z=5.266$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.90}
\figsetgrptitle{JADES-GN-189.13100+62.28684}
\figsetplot{figures/aastex_specfigs/spec_ID18651.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.13100+62.28684 at $z=5.267$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.91}
\figsetgrptitle{JADES-GN-189.12574+62.24596}
\figsetplot{figures/aastex_specfigs/spec_ID27297.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.12574+62.24596 at $z=5.267$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.92}
\figsetgrptitle{JADES-GN-189.12415+62.24222}
\figsetplot{figures/aastex_specfigs/spec_ID26772.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.12415+62.24222 at $z=5.268$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.93}
\figsetgrptitle{JADES-GN-189.11906+62.23624}
\figsetplot{figures/aastex_specfigs/spec_ID3804.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.11906+62.23624 at $z=5.269$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.94}
\figsetgrptitle{JADES-GN-189.11309+62.29239}
\figsetplot{figures/aastex_specfigs/spec_ID20485.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.11309+62.29239 at $z=5.270$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.95}
\figsetgrptitle{JADES-GN-189.12004+62.23867}
\figsetplot{figures/aastex_specfigs/spec_ID26307.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.12004+62.23867 at $z=5.271$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.96}
\figsetgrptitle{JADES-GN-189.15458+62.24755}
\figsetplot{figures/aastex_specfigs/spec_ID7473.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.15458+62.24755 at $z=5.272$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.97}
\figsetgrptitle{JADES-GN-189.11960+62.23855}
\figsetplot{figures/aastex_specfigs/spec_ID26305.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.11960+62.23855 at $z=5.274$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.98}
\figsetgrptitle{JADES-GN-189.15980+62.28796}
\figsetplot{figures/aastex_specfigs/spec_ID33394.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.15980+62.28796 at $z=5.274$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.99}
\figsetgrptitle{JADES-GN-189.26349+62.24229}
\figsetplot{figures/aastex_specfigs/spec_ID67088.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.26349+62.24229 at $z=5.283$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.100}
\figsetgrptitle{JADES-GN-189.23581+62.23532}
\figsetplot{figures/aastex_specfigs/spec_ID66305.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.23581+62.23532 at $z=5.285$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.101}
\figsetgrptitle{JADES-GN-189.09470+62.23936}
\figsetplot{figures/aastex_specfigs/spec_ID26460.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.09470+62.23936 at $z=5.292$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.102}
\figsetgrptitle{JADES-GN-189.05259+62.22990}
\figsetplot{figures/aastex_specfigs/spec_ID2222.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.05259+62.22990 at $z=5.294$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.103}
\figsetgrptitle{JADES-GN-189.14939+62.23187}
\figsetplot{figures/aastex_specfigs/spec_ID25527.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.14939+62.23187 at $z=5.295$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.104}
\figsetgrptitle{JADES-GN-189.09492+62.23948}
\figsetplot{figures/aastex_specfigs/spec_ID26462.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.09492+62.23948 at $z=5.295$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.105}
\figsetgrptitle{JADES-GN-189.11943+62.23994}
\figsetplot{figures/aastex_specfigs/spec_ID4902.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.11943+62.23994 at $z=5.295$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.106}
\figsetgrptitle{JADES-GN-189.08389+62.23713}
\figsetplot{figures/aastex_specfigs/spec_ID4051.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.08389+62.23713 at $z=5.296$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.107}
\figsetgrptitle{JADES-GN-189.12993+62.25251}
\figsetplot{figures/aastex_specfigs/spec_ID9100.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.12993+62.25251 at $z=5.296$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.108}
\figsetgrptitle{JADES-GN-189.12192+62.29101}
\figsetplot{figures/aastex_specfigs/spec_ID33818.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.12192+62.29101 at $z=5.297$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.109}
\figsetgrptitle{JADES-GN-189.12124+62.29358}
\figsetplot{figures/aastex_specfigs/spec_ID20827.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.12124+62.29358 at $z=5.297$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.110}
\figsetgrptitle{JADES-GN-189.14903+62.29347}
\figsetplot{figures/aastex_specfigs/spec_ID20794.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.14903+62.29347 at $z=5.297$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.111}
\figsetgrptitle{JADES-GN-189.25780+62.19996}
\figsetplot{figures/aastex_specfigs/spec_ID77966.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.25780+62.19996 at $z=5.299$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.112}
\figsetgrptitle{JADES-GN-189.22631+62.21190}
\figsetplot{figures/aastex_specfigs/spec_ID60083.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.22631+62.21190 at $z=5.311$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.113}
\figsetgrptitle{JADES-GN-189.11031+62.22544}
\figsetplot{figures/aastex_specfigs/spec_ID24940.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.11031+62.22544 at $z=5.344$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.114}
\figsetgrptitle{JADES-GN-189.11044+62.22533}
\figsetplot{figures/aastex_specfigs/spec_ID24939.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.11044+62.22533 at $z=5.346$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.115}
\figsetgrptitle{JADES-GN-189.25501+62.21625}
\figsetplot{figures/aastex_specfigs/spec_ID61639.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.25501+62.21625 at $z=5.348$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.116}
\figsetgrptitle{JADES-GN-189.21696+62.23168}
\figsetplot{figures/aastex_specfigs/spec_ID82594.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.21696+62.23168 at $z=5.354$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.117}
\figsetgrptitle{JADES-GN-189.17252+62.23584}
\figsetplot{figures/aastex_specfigs/spec_ID25944.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.17252+62.23584 at $z=5.355$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.118}
\figsetgrptitle{JADES-GN-189.12134+62.22823}
\figsetplot{figures/aastex_specfigs/spec_ID1844.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.12134+62.22823 at $z=5.356$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.119}
\figsetgrptitle{JADES-GN-189.06016+62.25651}
\figsetplot{figures/aastex_specfigs/spec_ID10155.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.06016+62.25651 at $z=5.360$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.120}
\figsetgrptitle{JADES-GN-189.06947+62.25945}
\figsetplot{figures/aastex_specfigs/spec_ID28904.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.06947+62.25945 at $z=5.362$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.121}
\figsetgrptitle{JADES-GN-189.04592+62.25416}
\figsetplot{figures/aastex_specfigs/spec_ID9636.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.04592+62.25416 at $z=5.362$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.122}
\figsetgrptitle{JADES-GN-189.16922+62.23847}
\figsetplot{figures/aastex_specfigs/spec_ID4452.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.16922+62.23847 at $z=5.418$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.123}
\figsetgrptitle{JADES-GN-189.12883+62.24377}
\figsetplot{figures/aastex_specfigs/spec_ID27048.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.12883+62.24377 at $z=5.420$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.124}
\figsetgrptitle{JADES-GN-189.21086+62.18661}
\figsetplot{figures/aastex_specfigs/spec_ID50989.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.21086+62.18661 at $z=5.421$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.125}
\figsetgrptitle{JADES-GN-189.18858+62.21303}
\figsetplot{figures/aastex_specfigs/spec_ID60534.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.18858+62.21303 at $z=5.426$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.126}
\figsetgrptitle{JADES-GN-189.04727+62.22963}
\figsetplot{figures/aastex_specfigs/spec_ID2176.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.04727+62.22963 at $z=5.428$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.127}
\figsetgrptitle{JADES-GN-189.26070+62.21626}
\figsetplot{figures/aastex_specfigs/spec_ID81060.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.26070+62.21626 at $z=5.432$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.128}
\figsetgrptitle{JADES-GN-189.15602+62.23872}
\figsetplot{figures/aastex_specfigs/spec_ID4535.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.15602+62.23872 at $z=5.435$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.129}
\figsetgrptitle{JADES-GN-189.12828+62.27297}
\figsetplot{figures/aastex_specfigs/spec_ID14285.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.12828+62.27297 at $z=5.435$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.130}
\figsetgrptitle{JADES-GN-189.04962+62.24405}
\figsetplot{figures/aastex_specfigs/spec_ID6269.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.04962+62.24405 at $z=5.442$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.131}
\figsetgrptitle{JADES-GN-189.05777+62.23927}
\figsetplot{figures/aastex_specfigs/spec_ID4725.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.05777+62.23927 at $z=5.443$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.132}
\figsetgrptitle{JADES-GN-189.08862+62.23949}
\figsetplot{figures/aastex_specfigs/spec_ID26483.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.08862+62.23949 at $z=5.443$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.133}
\figsetgrptitle{JADES-GN-189.14305+62.21142}
\figsetplot{figures/aastex_specfigs/spec_ID80036.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.14305+62.21142 at $z=5.446$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.134}
\figsetgrptitle{JADES-GN-189.18792+62.29720}
\figsetplot{figures/aastex_specfigs/spec_ID21821.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.18792+62.29720 at $z=5.450$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.135}
\figsetgrptitle{JADES-GN-189.15552+62.20012}
\figsetplot{figures/aastex_specfigs/spec_ID77708.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.15552+62.20012 at $z=5.456$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.136}
\figsetgrptitle{JADES-GN-189.15888+62.19685}
\figsetplot{figures/aastex_specfigs/spec_ID77270.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.15888+62.19685 at $z=5.456$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.137}
\figsetgrptitle{JADES-GN-189.15551+62.20002}
\figsetplot{figures/aastex_specfigs/spec_ID77706.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.15551+62.20002 at $z=5.457$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.138}
\figsetgrptitle{JADES-GN-189.06882+62.26887}
\figsetplot{figures/aastex_specfigs/spec_ID13172.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.06882+62.26887 at $z=5.470$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.139}
\figsetgrptitle{JADES-GN-189.23458+62.19048}
\figsetplot{figures/aastex_specfigs/spec_ID76044.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.23458+62.19048 at $z=5.484$.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{A1.140}
\figsetgrptitle{JADES-GN-189.14849+62.21166}
\figsetplot{figures/aastex_specfigs/spec_ID80185.pdf}
\figsetgrpnote{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.14849+62.21166 at $z=5.490$.}
\figsetgrpend

\figsetend
\begin{figure}
\figurenum{A1}
\plotone{figures/aastex_specfigs/spec_ID15254.pdf}
\caption{NIRCam images, 2D and 1D grism spectra of JADES-GN-189.09098+62.27600 at $z=5.126$. The upper-left panel shows the 1\farcs2$\times$1\farcs2 F444W--F277W--F150W RGB thumbnail. Images are rotated to align with the dispersion direction. The upper-right panel shows the continuum-subtracted 2D spectrum around the \ha\ emission line detection, indicated by the solid red line. The lower-right panel shows the optimally extracted 1D spectrum with the best-fit Gaussian profile indicated by the solid red line. The name and confirmed spectroscopic redshift are given in the lower-right panel for each galaxy. The complete figure set (140 images) is available in the online journal.}
\label{fig:apd_spec}
\end{figure}


==> author_list.tex <==
\author[0000-0001-7673-2257]{Zhiyuan Ji}
\affiliation{Steward Observatory, University of Arizona, 933 N. Cherry Ave., Tucson, AZ 85721, USA}

\author[0000-0002-4271-0364]{Brant Robertson}
\affiliation{Department of Astronomy and Astrophysics, University of California, Santa Cruz, 1156 High Street, Santa Cruz, CA 95064, USA}

\author[0000-0002-8224-4505]{Sandro Tacchella}
\affiliation{Kavli Institute for Cosmology, University of Cambridge, Madingley Road, Cambridge, CB3 0HA, UK}
\affiliation{Cavendish Laboratory, University of Cambridge, 19 JJ Thomson Avenue, Cambridge, CB3 0HE, UK"}

\author[0000-0003-0215-1104]{William M.\ Baker}
\affiliation{Kavli Institute for Cosmology, University of Cambridge, Madingley Road, Cambridge, CB3 0HA, UK}
\affiliation{Cavendish Laboratory, University of Cambridge, 19 JJ Thomson Avenue, Cambridge, CB3 0HE, UK}

\author[0000-0003-0883-2226]{Rachana Bhatawdekar}
\affiliation{European Space Agency (ESA), European Space Astronomy Centre (ESAC), Camino Bajo del Castillo s/n, 28692 Villanueva de la Cañada, Madrid, Spain}
\affiliation{European Space Agency, ESA/ESTEC, Keplerlaan 1, 2201 AZ Noordwijk, NL}

\author[0000-0003-4109-304X]{Kristan Boyett}
\affiliation{School of Physics, University of Melbourne, Parkville 3010, VIC, Australia}
\affiliation{ARC Centre of Excellence for All Sky Astrophysics in 3 Dimensions (ASTRO 3D), Australia}

\author[0000-0002-8651-9879]{Andrew J.\ Bunker}
\affiliation{Department of Physics, University of Oxford, Denys Wilkinson Building, Keble Road, Oxford OX1 3RH, UK}

\author[0000-0003-3458-2275]{Stephane Charlot}
\affiliation{Sorbonne Universit\'e, CNRS, UMR 7095, Institut d'Astrophysique de Paris, 98 bis bd Arago, 75014 Paris, France}

\author[0000-0002-7636-0534]{Jacopo Chevallard}
\affiliation{Department of Physics, University of Oxford, Denys Wilkinson Building, Keble Road, Oxford OX1 3RH, UK}

\author[0000-0002-9551-0534]{Emma Curtis-Lake}
\affiliation{Centre for Astrophysics Research, Department of Physics, Astronomy and Mathematics, University of Hertfordshire, Hatfield AL10 9AB, UK}

\author[0000-0002-2929-3121]{Daniel J.\ Eisenstein}
\affiliation{Center for Astrophysics $|$ Harvard \& Smithsonian, 60 Garden St., Cambridge MA 02138 USA}

\author[0000-0002-9708-9958]{A.\ Lola Danhaive}
\affiliation{Kavli Institute for Cosmology, University of Cambridge, Madingley Road, Cambridge, CB3 0HA, UK}
\affiliation{Cavendish Laboratory, University of Cambridge, 19 JJ Thomson Avenue, Cambridge, CB3 0HE, UK}

\author[0000-0002-4781-9078]{Christa DeCoursey}
\affiliation{Steward Observatory, University of Arizona, 933 N. Cherry Ave., Tucson, AZ 85721, USA}

\author[0000-0002-6221-1829]{Jianwei Lyu}
\affiliation{Steward Observatory, University of Arizona, 933 N. Cherry Avenue, Tucson, AZ 85721, USA}

\author[0000-0002-4985-3819]{Roberto Maiolino}
\affiliation{Kavli Institute for Cosmology, University of Cambridge, Madingley Road, Cambridge, CB3 OHA, UK}
\affiliation{Cavendish Laboratory - Astrophysics Group, University of Cambridge, 19 JJ Thomson Avenue, Cambridge, CB3 OHE, UK}
\affiliation{Department of Physics and Astronomy, University College London, Gower Street, London WC1E 6BT, UK}

\author[0000-0001-9276-7062]{Lester Sandles}
\affiliation{Kavli Institute for Cosmology, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK}
\affiliation{Cavendish Laboratory, University of Cambridge, 19 JJ Thomson Avenue, Cambridge CB3 0HE, UK}

\author[0000-0003-4702-7561]{Irene Shivaei}
\affiliation{Steward Observatory, University of Arizona, 933 N. Cherry Ave., Tucson, AZ 85721, USA}

\author[0000-0003-4891-0794]{Hannah \"Ubler}
\affiliation{Kavli Institute for Cosmology, University of Cambridge, Madingley Road, Cambridge, CB3 0HA, UK} 
\affiliation{Cavendish Laboratory, University of Cambridge, 19 JJ Thomson Avenue, Cambridge, CB3 0HE, UK.}

\author[0000-0002-4201-7367]{Chris Willott}
\affiliation{NRC Herzberg, 5071 West Saanich Rd, Victoria, BC V9E 2E7, Canada}

\author[0000-0002-7595-121X]{Joris Witstok}
\affiliation{Kavli Institute for Cosmology, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK}
\affiliation{Cavendish Laboratory, University of Cambridge, 19 JJ Thomson Avenue, Cambridge CB3 0HE, UK}


